Evolutionary Variational Optimization of Generative Models

We combine two popular optimization approaches to derive learning algorithms for generative models: variational optimization and evolutionary algorithms. The combination is realized for generative models with discrete latents by using truncated posteriors as the family of variational distributions. The variational parameters of truncated posteriors are sets of latent states. By interpreting these states as genomes of individuals and by using the variational lower bound to define a fitness, we can apply evolutionary algorithms to realize the variational loop. The used variational distributions are very flexible and we show that evolutionary algorithms can effectively and efficiently optimize the variational bound. Furthermore, the variational loop is generally applicable ("black box") with no analytical derivations required. To show general applicability, we apply the approach to three generative models (we use noisy-OR Bayes Nets, Binary Sparse Coding, and Spike-and-Slab Sparse Coding). To demonstrate effectiveness and efficiency of the novel variational approach, we use the standard competitive benchmarks of image denoising and inpainting. The benchmarks allow quantitative comparisons to a wide range of methods including probabilistic approaches, deep deterministic and generative networks, and non-local image processing methods. In the category of "zero-shot" learning (when only the corrupted image is used for training), we observed the evolutionary variational algorithm to significantly improve the state-of-the-art in many benchmark settings. For one well-known inpainting benchmark, we also observed state-of-the-art performance across all categories of algorithms although we only train on the corrupted image. In general, our investigations highlight the importance of research on optimization methods for generative models to achieve performance improvements.

==> fig/bars/app_bscssscBars.tex <==
\newcommand\widthL{5cm}
\newcommand\widthM{0.8cm}
\newcommand\spaceXSubplotLabel{0.4cm}
\newcommand\spaceYSubplotLabel{0.16cm}
\newcommand\SubplotLabelStyle{\Large \bf}
\newcommand\LineWidth{2pt}
\newcommand\spaceyLM{0.5cm}
\newcommand\spacexLM{0.1cm}
\newcommand\spaceMM{-0.2cm}
\newcommand\spaceMMgt{0.1cm}
\newcommand\spaceLabelLabel{0.05cm}
\newcommand\spaceXLabelLabel{-1.1cm}
\newcommand\spaceLabelY{-0.35cm}
\newcommand\spaceLabelX{-0.6cm}
\newcommand\spaceLabelXb{-0.75cm}
\newcommand\spaceLabelXc{-0.85cm}
\newcommand\LabelSize{\scriptsize}

\begin{minipage}[t]{0.32\textwidth}
\begin{tikzpicture}
    \newcommand\respath{fig/bars/bsc/19606708}
    \node(l) at (0,0) {\includegraphics[width=\widthL]{\respath_sigma.pdf}};
    \node[above right = \spaceYSubplotLabel and \spaceXSubplotLabel of l.north west, align=left, anchor = west](ll) {{\SubplotLabelStyle BSC}};    
\end{tikzpicture}
\end{minipage}
\hspace{0.04cm}
\begin{minipage}[t]{0.6\textwidth}
\begin{tikzpicture}
    \newcommand\respath{fig/bars/sssc/19606908}
    \node(l) at (0,0) {\includegraphics[width=\widthL]{\respath_mu.pdf}};
    \node[above left = 0.4 and -0.35 of l.north west](line_top) {};
    \node[below = 4.0 of line_top](line_bottom) {};
    \draw[draw=black,line width=\LineWidth] (line_top) to (line_bottom);
    \node[below right = \spaceyLM and \spacexLM of l.north east] (psi1) {\includegraphics[width=\widthM]{\respath_psisq_iter0.pdf}};
    \node[right = \spaceMM of psi1] (psi2) {\includegraphics[width=\widthM]{\respath_psisq_iter2.pdf}};
    \node[right = \spaceMM of psi2] (psi3) {\includegraphics[width=\widthM]{\respath_psisq_iter5.pdf}};
    \node[right = \spaceMM of psi3] (psi4) {\includegraphics[width=\widthM]{\respath_psisq_iter300.pdf}};
    \node[right = \spaceMMgt of psi4] (psi5) {\includegraphics[width=\widthM]{\respath_psisq_gt.pdf}};
    \node[above left = \spaceLabelLabel and \spaceXLabelLabel of psi3, align=center](psi_label) {\LabelSize $\Psi$ @ Iterations};
    \node[above left = \spaceLabelY and \spaceLabelX of psi1](psi1_label) {\LabelSize 0};
    \node[above left = \spaceLabelY and \spaceLabelX of psi2](psi2_label) {\LabelSize 2};
    \node[above left = \spaceLabelY and \spaceLabelX of psi3](psi3_label) {\LabelSize 5};
    \node[above left = \spaceLabelY and \spaceLabelXb of psi4](psi4_label) {\LabelSize 300};
    \node[above left = \spaceLabelLabel and \spaceLabelXc of psi5](psi5_label) {\LabelSize $\Psi^\gen$};

    \node[below = 0.6cm of psi1] (sigmasq1) {\includegraphics[width=\widthM]{\respath_sigmasq_iter0.pdf}};
    \node[right = \spaceMM of sigmasq1] (sigmasq2) {\includegraphics[width=\widthM]{\respath_sigmasq_iter2.pdf}};
    \node[right = \spaceMM of sigmasq2] (sigmasq3) {\includegraphics[width=\widthM]{\respath_sigmasq_iter5.pdf}};
    \node[right = \spaceMM of sigmasq3] (sigmasq4) {\includegraphics[width=\widthM]{\respath_sigmasq_iter300.pdf}};
    \node[right = \spaceMMgt of sigmasq4] (sigmasq5) {\includegraphics[width=\widthM]{\respath_sigmasq_gt.pdf}};
    \node[above left = \spaceLabelLabel and \spaceXLabelLabel of sigmasq3, align=center](sigmasq_label) {\LabelSize $\Sigma$ @ Iterations};
    \node[above left = \spaceLabelY and \spaceLabelX of sigmasq1](sigmasq1_label) {\LabelSize 0};
    \node[above left = \spaceLabelY and \spaceLabelX of sigmasq2](sigmasq2_label) {\LabelSize 2};
    \node[above left = \spaceLabelY and \spaceLabelX of sigmasq3](sigmasq3_label) {\LabelSize 5};
    \node[above left = \spaceLabelY and \spaceLabelXb of sigmasq4](sigmasq4_label) {\LabelSize 300};
    \node[above left = \spaceLabelLabel and \spaceLabelXc of sigmasq5](sigmasq5_label) {\LabelSize $\Sigma^\gen$};

    \node[above right = \spaceYSubplotLabel and \spaceXSubplotLabel of l.north west, align=left, anchor = west](ll) {{\SubplotLabelStyle SSSC}};
\end{tikzpicture}
\end{minipage}

==> fig/genetic_operators/genetic_operators.tex <==
\begin{tikzpicture}[
    declare function={
        f(\x)=2+sin(deg(\x-2-0.2))+sin(deg(3*(\x-0.2)))/2+sin(deg(5*(\x-0.2)))/8 + sin(deg(7*(\x-0.2)))/28;        
    }
]

\begin{axis}[axis 
lines = middle,smooth,
height=4cm,
width=4cm,
xlabel = $\vec{s}$, 
% ylabel =$F\left(\vec{s}\right)$, 
% minor tick num =1, 
grid=none, 
no markers, 
xtick={2,3,4,5,6,7},
% xticklabels={,\ArrowUp,,,,\ArrowUp,,},
xticklabels={,$\vec{s}_a$,,,,$\vec{s}_b$,,},
every axis x label/.style={ at={(ticklabel* cs:1.05)}, anchor=west},
ytick={0},
every axis y label/.style={at={(ticklabel* cs:1.05)},anchor=south},
domain=1:8, 
enlargelimits = false,
]

\clip (axis cs:1.1,0.0) rectangle (axis cs:7.8,90);
\addplot [  
    domain=1:8,
    samples=300,
    line width=1pt,    
    mark=*,
    draw=black,    
] {f(x)} \closedcycle;
\addplot[color=black,mark size=2] coordinates {(3,0) (3,{f(3)})};
\addplot[color=black,mark size=2] coordinates {(7,0) (7,{f(7)})};
\end{axis}

\node(a) at (0.36\columnwidth,1.5){$\vec{s}_a:\left(1~\cdots~1~1\right)$};    
\node[below = 0cm of a](b){$\vec{s}_b:\left(0~\cdots~0~1\right)$};    
\node[right = 0.8cm of a](c){$\left(1~\cdots~0~1\right)$};    
\node[below = 0cm of c](d){$\left(0~\cdots~1~1\right)$};   

\node[above right = 0.0 cm and 3.5 cm of c.west](g){$\left(1~\cdots~0~1\right)$};   
\node[below = 0.6cm of g](h){$\left(0~\cdots~1~1\right)$};   
\node[above right= 0.1cm and -0.9cm of a] (e) {};
\node[below right= 0.1cm and -0.9cm of b] (f) {};
\path [->]
  (a.south east) edge node [above] {}  (c.south west);
\draw[dotted] (e) {} -- (f) {};

\node[above left= 0.8cm and 1.5cm of a] (j) {{\bf A) Parent selection}};
\node[below left = 0.3 and -0.5 of j.west,rotate=90](oo) {$\mathit{f}(\sVec;\yVec,\KKn_{g},\Theta)$};

\node[right= 2.8cm of j] (k) {{\bf B) Crossover}};
\node[right = 2.6cm of k] (l) {{\bf C) Mutation}};

\node[below left= -0.2cm and -0.45cm of g] (m) {};
\node[below left= 0.6cm and -0.45cm of g] (n) {};

\node[right= 0.7cm of m] (o) {};
\node[right= 0.7cm of n] (p) {};

\path [->]    
  (m) edge node [left] {$p_1$}  (n) %p(s_h=0\vert s_h=1)
  (o) edge node [right] {$p_0$}  (p);%p(s_h=1\vert s_h=0)

\end{tikzpicture}
